Quantum many-body scars in bipartite Rydberg arrays originate from hidden projector embedding

We study the nature of the ergodicity-breaking "quantum many-body scar" states that appear in the PXP model describing constrained Rabi oscillations. For a {wide class of bipartite lattices} of Rydberg atoms, we reveal that the nearly energy-equidistant tower of these states arises from the Hamiltonian's close proximity to a generalized projector-embedding form, a structure common to many models hosting quantum many-body scars. We construct a non-Hermitian, but strictly local extension of the PXP model hosting exact quantum scars, and show how various Hermitian scar-stabilizing extensions from the literature can be naturally understood within this framework. The exact scar states are obtained analytically as large spin states of explicitly constructed pseudospins. The quasi-periodic motion ensuing from the N\'eel state is finally shown to be the projection onto the Rydberg-constrained subspace of the precession of the large pseudospin.

==> files_not_used/deformation.tex <==
\subsection{A connection to the weakly broken Lie algebra and a systematic way to perturb the model}
It is known that certain types of perturbation stabilize the revival~\cite{turner_tower,nearly_su2,integrability,PhysRevResearch.2.033044,Kieran2020,Lin2020}. In this section, we rederive these terms and discuss them in terms of our island approach and the approximate SGA, following the argument of the broken lie algebra~\cite{Kieran2020}.

We start from the following observation: the PXP Hamiltonian is regarded as a sum of the ``spin raising" operator and ``spin lowering" operator by a unitary transformation $U\equiv\exp\left[i\pi/4\sum_j(-1)^jZ_j\right]$
\begin{equation}
    H=\frac{i}{\sqrt{2}}\left(U^\dag Q^\dag(\pi)U-U^\dag Q(\pi)U\right).
\end{equation}
We define the spin raising part as $S^+(\pi)$ and the lowering as $S^-(\pi)$. From this definition we can also define $z$-component of the spin operator $S^z(\pi)$ as $S^z(\pi)\equiv\left[S^+(\pi),S^-(\pi)\right]/2$. These spin operators $S^\pm(\pi)$ and $S^z(\pi)$ almost satisfy $SU(2)$ algebra allowing error terms.
\begin{equation}
    \left[S^z(\pi), S^\pm(\pi)\right]=\pm S^+(\pi)+\sum^6_{i=1}\delta_i^\pm,
\end{equation}
where
\begin{equation}
    \begin{aligned}
    \delta_1^\pm&=\frac{i}{2\sqrt{2}}\sum_jP_{j-1}X_jP_{j+1}\\
    \delta_2^\pm&=\frac{5i}{4\sqrt{2}}\sum_jP_{j-1}X_jP_{j+1}\left(Z_{j-2}+Z_{j+2}\right)\\
    \delta_3^\pm&=\mp\frac{1}{8}\sum_j(-1)^jZ_{j-3}P_{j-2}\left(X_{j-1}X_j+Y_{j-1}Y_j\right)P_{j+1}\\
    &\mp\frac{1}{8}\sum_j(-1)^jP_{j-1}\left(X_jX_{j+1}+Y_jY_{j+1}\right)P_{j+2}Z_{j+3}\\
    \delta_4^\pm&=\pm\frac{1}{2}\sum_j(-1)^jP_{j-1}Z_jP_{j+1}\left(Z_{j-2}+Z_{j+2}\right)\\
    \delta_5^\pm&=\mp\sum_j(-1)^jP_{j-1}X_jP_{j+1}X_{j+2}P_{j+3}\\
    \delta_6^\pm&=-\frac{i}{2\sqrt{2}}\sum_jP_{j-1}X_jP_{j+1}\left(Z_{j-2}P_{j+2}+P_{j-2}Z_{j+2}\right).
    \end{aligned}
\end{equation}
These terms lead to the following perturbation terms with parameters $\lambda_i (i=1, 2)$,
\begin{equation}\label{eq: perturbed}\begin{aligned}
    H'&=\sum_jP_{j-1}X_jP_{j+1}\\&+\lambda_1\sum_jP_{j-1}X_jP_{j+1}\big(Z_{j-2}+Z_{j+2}\big)\\
    &+\lambda_2\sum_jP_{j-1}X_jP_{j+1}\big(Z_{j-2}P_{j+2}+P_{j-2}Z_{j+2}\big)
    \end{aligned}
\end{equation}
Perturbations in Eq.\eqref{eq: perturbed} have been discussed Refs.~\cite{turner_tower,nearly_su2,integrability,PhysRevResearch.2.033044,Kieran2020,Lin2020} and as in Ref.~\cite{Kieran2020} we also reproduce perturbations which stabilize the revival in a systematic manner.

==> files_not_used/discussion.tex <==
We devote this section to point out important differences between our approach and previous studies, particularly Ref.~\cite{nearly_su2} and Ref.~\cite{magnon_condensation}.

First, we note that nearly $SU(2)$ algebra \cite{nearly_su2} is not included in our formalism although it apparently is by taking $\ket{\psi}=\ket{\mathbb{Z}_2}$. However, The reference state must be 

==> files_not_used/other_approach.tex <==
In this section, we compare our approach with other approaches that are nearly $SU(2)$ algebra[REF], proximity to the Lesanovsky model[REF], $\pi$-magnon condensation[REF], and matrix product state ansatz[REF]. We show that they are successful since each approach can somehow produce the FP state and the singlet on it. Here, we assume the PBC, i.e., $H_{\mr{PBC}}$.   
%\subsection{Particle-hole analogy}
%To make a connection to other approaches, we introduce an idea which is essentially the same as polarized fractional spin-$1/2$s. In Sec.~\ref{magnon}, we conclude that the scar states are understood as polarized pairs of fractional spin-$1/2$s on top of the VBS state. This means we take the reference state as the VBS state, and apply the operator that polarizes fractional spin-$1/2$s. However, we can also take the FP states as a reference state and apply the Hermitian conjugate of that operator, i.e., for $n<0$, 
%\begin{equation}
    %\ket*{S'_n}\equiv P_{\mr{Ryd}}\left(\sum_b(-1)^b\left(S_b^y+iS_b^z\right)\right)^{N-|n|}\ket*{\Phi_{\mr{FP}}^-},
%\end{equation}
%and for $n>0$,
%\begin{equation}
    %\ket*{S'_n}\equiv P_{\mr{Ryd}}\left(\sum_b(-1)^b\left(S_b^y-iS_b^z\right)\right)^{N-n}\ket*{\Phi_{\mr{FP}}^+}.
%\end{equation}
%Physically, we start from the ferromagnetic FP state, and by acting $\sum_b(-1)^b\left(S_b^y\pm iS_b^z\right)$, a pair of neighboring fractional spin-$1/2$s forms the dimer. Although $\ket*{S_n}\not=\ket*{S'_n}$ for a general $n$ and the squared overlap between $\ket*{\mc{S}_n}$ and $\ket*{S'_n}$ is worse than one between $\ket*{\mc{S}_n}$ and $\ket*{S_n}$, $\ket*{S_n}$ and $\ket*{S'_n}$ are close particularly when $n$ is close to $\pm N$ (the dimers are ``dilute"), and $\ket*{S'_n}$ approximates the scar state relatively accurately (Fig.\ref{fig:magnon_results}).

%This idea is similar to electrons in a solid: when they are in an almost fulled band, we rather take a completely filled band as a reference state, and regard the absence of electrons as excitations, i.e., holes. Here we can regard the dimer as an excitation if the reference state is the FP state.  
\subsection{Nearly $SU(2)$ algebra and forward scattering approximation}
\label{sec:nearly su2}
%introduction

We briefly review the nearly $SU(2)$ algebra and the forward scattering approximation (FSA) in the PXP model. $H_{\mr{PBC}}$ is split into the ``raising" operator $H^+$ and the ``lowering" operator $H^-$: in the original spin-$1/2$ representation, they are defined as 
\begin{equation}
    H^\pm\equiv\sum_{n=1}^{2N}\left(P_{2n-1}\sigma^\pm_{2n}P_{2n+1}+P_{2n-2}\sigma^\mp_{2n-1}P_{2n}\right),
\end{equation}
where $\sigma^+\equiv\dyad{\uparrow}{\downarrow}$ and $\sigma^-\equiv\dyad{\downarrow}{\uparrow}$. From these operators, we can also define ``$z$-component" by standard $SU(2)$ algebra:
\begin{equation}\begin{split}
    H^z&\equiv\frac{1}{2}\left[H^+,H^-\right]\\
    &=\frac{1}{2}\sum_n\left(P_{2n-1}Z_{2n}P_{2n+1}-P_{2n-2}Z_{2n-1}P_{2n}\right).
    \end{split}
\end{equation}
These operators satisfy algebra similar to that of $SU(2)$, i.e., $[H^z,H^+]\cong\Delta H^+$ with a coefficient $\Delta$ in some subspace. This subspace is constructed as follows: the N\'{e}el state $\ket{\mb{Z}_2}\equiv\ket{\uparrow\downarrow\uparrow\cdots}$ is regarded as the lowest weight state as it is annihilated by $H^-$. From the lowest weight state, we obtain new states by repeatedly acting $H^+$, i.e., $\ket{k}\propto(H^+)^k\ket{\mb{Z}_2}$. This process is terminated when $k=2N+1$, as $(H^+)^{2N}\ket{\mb{Z}_2}\propto\ket{\downarrow\uparrow\downarrow\cdots}\equiv\ket{\mb{Z}'_2}$ and $H^+\ket{\mb{Z}'_2}=0$. In this way, we obtain $2N+1$ linearly independent vectors that span the subspace. %Here we refer to this subspace as the FSA subspace $\mb{V}_{\mr{FSA}}$, i.e., 
%\begin{equation}
    %\mb{V}_{\mr{FSA}}\equiv\mr{span}\left\{\left(H^+\right)^k\ket{\mb{Z}_2};0\leq k\leq 2N\right\}.
%\end{equation}
%We further define an extended FSA subspace $\widetilde{\mb{V}}_{\mr{FSA}}$ as
%\begin{equation}
    %\widetilde{\mb{V}}_{\mr{FSA}}\equiv\mr{span}\left\{\left(H^+\right)^{k}\right\}
%\end{equation}
%We also define a similar subspace defined by $\ket{\Phi_{\mr{FP}}^\pm}$, $Q^\dag$, and $Q$ as follows:
%\begin{equation}\begin{split}
    %\mb{V}_{\mr{mag}}&\equiv\left\{\left(Q^\dag\right)^k\ket{\Phi_{\mr{VBS}}};0\leq k\leq N\right\}\\
    %&\cup\Big\{Q^k\ket{\Phi_{\mr{VBS}}};1\leq k\leq N\Big\}.
%\end{split}
%\end{equation}

We propose a possible connection between our approach and this approach. In the spin-$1$ basis, $H^+$ is expressed as
\begin{equation}
    \begin{split}
        H^+&=\frac{1}{\sqrt{2}}\sum_n\left(S_{2n-1}^++S_{2n}^-\right)\\&-\sum_n\left(\dyad{-,-}{0,-}-\dyad{-,0}{-,-}\right)_{2n-1,2n}\\
        &-\sum_n\left(\dyad{+,+}{0,+}+\dyad{+,0}{+,+}\right)_{2n,2n+1}.
    \end{split}
\end{equation}
One can find that the FP states $\ket*{\Phi_{\mr{FP}}^\pm}$ in the constrained subspace can be approximately constructed by $H^+$ and $\ket{\mb{Z}_2}$: the FP state is expressed as 
\begin{equation}
    \ket*{\Phi_{\mr{FP}}^\pm}=\frac{1}{2^N}\left[\pm\sum_n\left(S_{2n-1}^++S_{2n}^-\right)\right]\ket*{\mb{Z}_2},
\end{equation}
where $\ket*{\mb{Z}_2}\equiv\ket*{-+-+\cdots}$ is the N\'{e}el state in the spin-$1$ representation. Note that $H^+$ is re-written in the spin-$1$ basis as
\begin{equation}
    \begin{split}
        H^+&=\frac{1}{\sqrt{2}}\sum_n\left(S_{2n-1}^++S_{2n}^-\right)\\
        &-\sum_n\big(\dyad{+,+}{0,+}+\dyad{+,0}{+,+}\big)_{2n-1,2n}\\
        &-\sum_n\big(\dyad{-,-}{0,-}+\dyad{-,0}{-,-}\big)_{2n,2n+1},
    \end{split}
\end{equation}
where the second and the third lines impose the Rydberg constraint.

Although a naive expectation that $e^{\pm\sqrt{2}H^+}\ket*{\mb{Z}_2}\propto P_{\mr{Ryd}}\ket*{\Phi_{\mr{FP}}^\pm}$ is not true as $S_b^\pm$ does not commute with $P_{\mr{Ryd}}$, they are still close to each other. Indeed, the squared overlap between $\ket*{\mc{S}_{\pm N}}$ and $e^{\pm\sqrt{2}H^+}\ket*{\mb{Z}_2}$ is $0.8722$ for $N=10$. 

We can also expect that states that are close to $\ket{S_{\pm(N-1)}}$ can be created in a similar manner. Up to irrelevant phase factor, $\ket*{S_{\pm(N-1)}}$ are written as
\begin{equation}
    \ket*{S_{\pm(N-1)}}=P_{\mr{Ryd}}\sum_{b=1}^N(-1)^b\ket*{D^\pm_b},
\end{equation}
where 
\begin{equation}
    \begin{split}
        \ket*{D_b^+}&\equiv\left(\bigotimes_{b'}\ms{S}_{b'}\right)\bigotimes_{b''\not=b}\ket{\rightarrow}_{b'',\mr{R}}\ket{\rightarrow}_{b''+1,\mr{L}}\\
        &\otimes\frac{1}{\sqrt{2}}\left(\ket*{\uparrow}_{b,\mr{R}}\ket*{\downarrow}_{b+1,\mr{L}}-\ket*{\downarrow}_{b,\mr{R}}\ket*{\uparrow}_{b+1,\mr{L}}\right)\\
        \ket*{D_b^-}&\equiv\left(\bigotimes_{b'}\ms{S}_{b'}\right)\bigotimes_{b''\not=b}\ket{\leftarrow}_{b'',\mr{R}}\ket{\leftarrow}_{b''+1,\mr{L}}\\
        &\otimes\frac{1}{\sqrt{2}}\left(\ket*{\uparrow}_{b,\mr{R}}\ket*{\downarrow}_{b+1,\mr{L}}-\ket*{\downarrow}_{b,\mr{R}}\ket*{\uparrow}_{b+1,\mr{L}}\right).
    \end{split}
\end{equation}
Namely, $\ket{D_b^\pm}$ is a configuration where a dimer is placed at a bond between sites $b$ and $b+1$ on the background of the polarized spins. We show that $\sum_b(-1)^b\ket{D_b^\pm}$ is constructed by $\sum_nS_{2n-1}^++S^-_{2n}$ and $\ket{\mb{Z}_2}$. Note that this statement implies our expectation, as $H^+$ is regarded as $\sum_bS_{2n-1}^++S_{2n}^-$ projected onto the constrained subspace. A straightforward calculation yields
\begin{widetext}
\begin{equation}
    \begin{split}
        \sum_b(-1)^b\ket*{D_b^+}&=\frac{1}{2^N}\sum_n\exp\left[-\frac{1}{2}\left(S_{2n-1}^-\right)^2+S_{2n}^++\sum_{n'\not=n}\left(S^-_{2n'-1}+S_{2n'}^+\right)\right]\ket{\mb{Z}_2}\\
        &+\frac{1}{2^N}\sum_n\exp\left[S_{2n-1}^+-\frac{1}{2}\left(S_{2n}^+\right)^2+\sum_{n'\not=n}\left(S^-_{2n'-1}+S_{2n'}^+\right)\right]\ket*{\mb{Z}_2}\\
        \sum_b(-1)^b\ket*{D_b^-}&=\frac{1}{2^N}\sum_n\exp\left[-\frac{1}{2}\left(S_{2n-1}^-\right)^2-S_{2n}^+-\sum_{n'\not=n}\left(S^-_{2n'-1}+S_{2n'}^+\right)\right]\ket{\mb{Z}_2}\\
        &+\frac{1}{2^N}\sum_n\exp\left[-S_{2n-1}^+-\frac{1}{2}\left(S_{2n}^+\right)^2-\sum_{n'\not=n}\left(S^-_{2n'-1}+S_{2n'}^+\right)\right]\ket*{\mb{Z}_2}.
    \end{split}
\end{equation}
\end{widetext}
Operators in this equation are mutually commutable and invariant under any permutation. Therefore, they must be a function of $\sum_nS_{2n-1}^-+S_{2n}^+$.   
%singlet can be created by e^(H^+^2)|Z2>!

This consideration implies that we can create dimers and the FP state by acting $H^+$ on $\ket*{\mb{Z}_2}$, which are essential ingredients of the scar states. Therefore, the subspace spanned by $\left\{\ket{k}\right\}$ could include them. 
\subsection{Lesanovsky model}
It is pointed out in Ref.[REF] that the ground state of the PXP model can be approximated by the ground state of the Lesanovsky model[REF], which is defined as 
\begin{equation}
    H_{\mr{Les}}=\sum_{i=1}^{2N}P_{i-1}\left(X_i+\frac{1}{z}n_j+zP_j\right)P_{i+1},
\end{equation}
where $z$ is a parameter and $n_i\equiv\dyad{\uparrow}_i$. The ground state of $H_{\mr{Les}}$ is exactly known for an arbitrary $z$ and it is
\begin{equation}
    \ket{z}=\exp\left[-z\sum_{j=1}^{2N}P_{j-1}\sigma_j^+P_{j+1}\right]\bigotimes_{i=1}^{2N}\ket{\downarrow}_i.
\end{equation}
In Ref.[REF], the ground state of the PXP model and $\ket{z}$ are compared and the squared overlap between them becomes the largest when $z\cong0.65$ for $N=13$. Here we show this correspondence is explained within our framework.

In the spin-$1$ basis, $\ket{z}$ is written as
\begin{equation}
    \ket{z}=P_{\mr{Ryd}}\exp\left[-z\sum_{b=1}^N\left(\dyad{+}{0}+\dyad{-}{0}\right)_b\right]\bigotimes_{b'=1}^N\ket{0}_{b'}.
\end{equation}
When $z=1/\sqrt{2}\cong0.71$, one can show that $\ket{z=1/\sqrt{2}}=P_{\mr{Ryd}}\ket*{\Phi_{\mr{FP}}^-}$, which is a good approximation to the ground state with the squared overlap about $0.96$ for $N=10$, as seen in Sec.\ref{subsec:|S_n>}. While the optimal value of $z$ for $N=10$ is about $0.65$ with the squared overlap around $0.98$, it is concluded that difference between $\ket*{z\cong0.65}$ and $\ket*{z=1/\sqrt{2}}$ is inessential. Therefore, one can understand $\ket*{z\cong0.65}$ as a slightly modified FP state.
\subsection{$\pi$-magnon condensation}
The scar states in the PXP model are also understood as the so-called ``$\pi$-magnon"[REF]. As its name suggests, the scar states are assumed to be quasi-particle-like excitations that are excited by the creation operator $S^\pm_\pi$: in the original spin-$1/2$ basis, it is defined as
\begin{equation}
    S^\pm_\pi\equiv\frac{1}{2}\sum_{i=1}^{2N}(-1)^i\big(Z_i\pm i\alpha P_{i-1}Y_iP_{i+1}\big),
\end{equation}
where $\alpha$ is a parameter. The parameter $\alpha$ is variationally optimized so that $S^\pm_\pi$ creates and annihilates the first excited state from the ground state $\ket{\Phi_{\mr{GS}}}$ which is also determined variationally. Using the optimal $S_\pi^\pm$, the $n$-magnon state $\ket{n}$ is defined as $\ket{n}\equiv\mc{N}^{-1}\left(S_\pi^+\right)^n\ket{\Phi_{\mr{GS}}}$ with a normalization factor $\mc{N}$. Also, the particle-hole pair of such states, denoted as $\ket*{\widetilde{n}}$, is defined as $\ket*{\widetilde{n}}\equiv\mc{N}^{-1}\left(S_\pi^-\right)^n\ket{\Phi_{\mr{CE}}}$ where $\ket{\Phi_{\mr{CE}}}$ is the ceiling state and $\mc{N}$ is a normalization factor. These magnon states span a subspace, and it is shown that this subspace captures the scar states relatively well. %Note that the magnon states are not approximate states of the scar states, and the subspace includes states other than the scar states. 

We propose a possible connection to our approach. In the spin-$1$ basis, the creation operator is re-written as
\begin{equation}\label{eq:S_pi^pm}\begin{split}
    S_\pi^\pm&=\pm i\frac{\alpha}{\sqrt{2}}\sum_b(-1)^b\big(S_b^y\pm iS_b^z\big)\\&+\left(\frac{\alpha}{\sqrt{2}}-\frac{1}{2}\right)\sum_b(-1)^bS_b^z\\
    &+\frac{\alpha}{\sqrt{2}}\sum_n\big(\dyad{T_{2,2}}{T_{1,1}}-\dyad{T_{1,1}}{T_{2,2}}\big)_{2n-1,2n}\\
    &-\frac{\alpha}{\sqrt{2}}\sum_n\big(\dyad{T_{2,-2}}{T_{1,-1}}-\dyad{T_{1,-1}}{T_{2,-2}}\big)_{2n,2n+1}.
    \end{split}
\end{equation}
Note that $S_\pi^{\pm}$ contains $\sum_b(-1)^b(S_b^y\pm iS_b^z)$, which is essential to create the dimers from polarized spins. The third and the fourth lines of Eq.\eqref{eq:S_pi^pm} impose the Rydberg constraint. Therefore, in total this operator create polarized spins with the momentum $\pi$, which is qualitatively the same as our ansatz $\ket{S'_n}$. However the second line of Eq.\eqref{eq:S_pi^pm} causes a deviation so that the $\pi$-magnon itself is a worse approximation to the scar state, compared with our approach. Nevertheless, $\ket*{n}$ (and $\ket*{\wtil{n}}$) can still capture the scar state $\ket*{\mc{S}_n}$ to some extent due to the first term of Eq.\eqref{eq:S_pi^pm}. Note that in the fractional spin-$1/2$ representation, the second line is written as $\sum_b(-1)^bS_b^z\left(\bigotimes_{b'=1}^N\ms{S}_{b'}\right)=\left(\bigotimes_{b'=1}^N\ms{S}_{b'}\right)\sum_b(-1)^b\left(S_{b,\mr{L}}^z+S_{b,\mr{R}}^z\right)$ and $S_{b,\mr{L/R}}^z$ only flips the polarization, i.e., $S_{b,\mr{L/R}}^z\ket{\rightarrow}=\ket{\leftarrow}/2$ and $S_{b,\mr{L/R}}^z\ket{\leftarrow}=\ket{\rightarrow}/2$. This implies that the second line of Eq.\eqref{eq:S_pi^pm} does not ruin the structure of the scar state (dimers + polarized spins) altogether.
\subsection{Matrix product state ansatz}
In Ref.[REF], it is claimed that the scar states can be understood as a quasi-particle-like excitation on top of the VBS state, and the ansatz wave function $\ket*{M_n}$ for the scar states $\ket*{\mc{S}_n}$ is given as a matrix product state (MPS) with two variational parameters $\mu_1$ and $\mu_2$. Those paramters are optimized by minimizing the variance of $H_{\mr{PBC}}$, i.e., $\ev{H_{\mr{PBC}}^2}{M_{-1}}-\ev{H_{\mr{PBC}}}{M_{-1}}^2$. Although $\ket*{M_n}$ is a MPS, we can define the creation operator $Q^\dag_{\mr{MPS}}$ such that $\ket*{M_{-1}}=Q^\dag_{\mr{MPS}}\ket*{\Phi_{\mr{VBS}}}$: in the spin-$1$ basis, it is
\begin{widetext}
\begin{equation}\label{eq:Q_MPS}
    \begin{split}
        Q^\dag_{\mr{MPS}}&=\sum_b(-1)^b\left(\frac{1}{\sqrt{2}}\big(\dyad{0}{-}-\dyad{0}{+}\big)_b-\mu_2\big(\dyad{+}{0}-\dyad{-}{0}\big)_b-\frac{\mu_1}{\sqrt{2}}S_b^z\right)\\
        &+\sum_n\left(\sqrt{2}\mu_2\dyad{T_{2,2}}{T_{1,1}}+\frac{\mu_2}{\sqrt{2}}\dyad{T_{2,1}}{T_{2,-2}}-\frac{\mu_2}{2}\dyad{0,+}{-,+}-\frac{\mu_2}{2}\dyad{+,0}{+,-}\right)_{2n-1,2n}\\
        &+\sum_n\left(-\sqrt{2}\mu_2\dyad{T_{2,-2}}{T_{1,-1}}+\frac{\mu_2}{\sqrt{2}}\dyad{T_{2,-1}}{T_{2,2}}-\frac{\mu_2}{2}\dyad{-,0}{-,+}-\frac{\mu_2}{2}\dyad{0,-}{+,-}\right)_{2n,2n+1}.
    \end{split}
\end{equation}
\end{widetext}
For $N=12$, the optimal values are $\mu_1\cong-1.087$ and $\mu_2\cong-0.6344$[REF]. Note that the first line of Eq.\eqref{eq:Q_MPS} becomes $i\sum_b(-1)^b(S_b^y-iS_b^z)$ when $\mu_1=-\sqrt{2}$ and $\mu_2=-1/\sqrt{2}$, which are not far from the optimal values. Therefore, $Q^\dag_{\mr{MPS}}$ essentially creates a pair of polarized spin-$1/2$s in $-x$-direction with some corrections described in the second and the third lines of Eq.\eqref{eq:Q_MPS}, which is compatible with the fact that $\ket*{M_1}$ is obtained by $\mu_1\rightarrow-\mu_1$, corresponding to $i\sum_b(-1)^b(S_b^y+iS_b^z)$. For $N=10$, we confirm that the optimal values are $\mu_1=-0.9308$ and $\mu_2=-0.4548$, which are not close to $\mu_1=-\sqrt{2},\mu_2=-1/\sqrt{2}$. However, the squared overlap between $\ket{M_{-1}}$ with $\mu_1=-\sqrt{2}, \mu_2=-1/\sqrt{2}$ and $\ket*{\mc{S}_{-1}}$ is $0.5799$ while one between one with the optimal values and $\ket*{\mc{S}_{-1}}$ is $0.5891$. This means that the difference is just quantitative from the viewpoint of approximating $\ket{\mc{S}_{-1}}$.        
%check numerically that mu_1, mu_2 are essentially sqrt(2), 1/sqrt(2) and difference between the optimal value and these values are small  

==> files_not_used/other_models.tex <==
In this section, we will show that the basic structure Eq.\eqref{eq:basic scheme} appears in the spin-$1$ XY model~\cite{tos_xy}, the spin-$1/2$ domain-wall conserving model~\cite{tos_exact_2}, and the Affleck-Kennedy-Lieb-Tasaki (AKLT) model~\cite{Affleck1987}. 
\subsection{Spin-1 XY model}
The spin-$1$ XY model is understood as an anisotropic Heisenberg interaction with the easy-plane anisotropy. This model is defined on the square lattice in an arbitrary dimension, and hosts the scar states~\cite{tos_xy}. Although a decomposition of the Hamiltonian into the spectrum-generating term and local annihilators is already known for this model, we can re-derive it in a way that can be applicable to other models.  
%\subsubsection{One dimensional case}

When the system is one dimensional, the model Hamiltonian is given as follows:
\begin{equation}\label{eq:one dim XY}
    H_{\mr{XY}}=J\sum_i\left(S_i^xS_{i+1}^x+S_i^yS_{i+1}^y\right)+D\sum_i\left(S_i^z\right)^2+h\sum_iS_i^z,
\end{equation}
where $S^\alpha (\alpha=x,y,z)$ is a spin operator with $S=1$, and we assume periodic boundary condition (PBC), identifying $S^\alpha_{i+N}=S^\alpha_i(\alpha=x,y,z)$. Here, we consider one dimensional case for simplicity. But an extension to higher dimension is straightforward as we will see. 
The scar states are generated by a ``creation" operator $Q_{\mr{XY}}^\dag\equiv\sum_i(-1)^i\left(S_i^+\right)^2$ acting on the ferromagnetic state $\ket{\Omega}\equiv\bigotimes_i\ket{-}_i$. The scar state, denoted as $\ket*{S_n^{\mr{XY}}}\equiv\mc{N}_n^{-1}\left(Q^\dag_{\mr{XY}}\right)^\dag\ket{\Omega}$ has an energy $E_n=(2n-N)h+ND$. The absence of $J$ in $E_n$ implies that the first term in Eq.\eqref{eq:one dim XY} annihilates the scar states. In fact, it is explicitly stated that each term, i.e., $S_i^xS_{i+1}^x+S_i^yS_{i+1}^y$ annihilates all scar states in Ref.~\cite{tos_xy}. Here, we show it in a different way: it is decomposed as 
\begin{equation}\label{eq:SxSx+SySy}\begin{split}
    S_i^xS_{i+1}^x+S_i^yS_{i+1}^y&=2\left(P_{i,i+1}^{(2,2)}+P_{i,i+1}^{(2,-2)}+P_{i,i+1}^{(1,0)}-1\right)\\&+3\left(P_{i,i+1}^{(2,1)}+P_{i,i+1}^{(2,0)}+P_{i,i+1}^{(2,-1)}\right)\\&+P_{i,i+1}^{(1,1)}+P_{i,i+1}^{(1,-1)}\\+\frac{3}{4}&\left(\ket{T_{2,0}}+\ket{T_{0,0}}\right)\left(\bra{T_{2,0}}+\bra{T_{0,0}}\right)_{i,i+1},
    \end{split}
\end{equation}
where $P_{i,j}^{(S,M)}$ is a projection operator onto a composite spin state $\ket*{T_{S,M}}$ such that $(\bm{S}_i+\bm{S}_j)^2\ket*{T_{S,M}}=S(S+1)\ket*{T_{S,M}}$ and $S_i^z+S_j^z\ket*{T_{S,M}}=M\ket*{T_{S,M}}$.

The scar states are annihilated by $P_{i,i+1}^{(2,2)}+P_{i,i+1}^{(2,-2)}+P_{i,i+1}^{(1,0)}-1$, and by any other projection operator appearing in Eq.\eqref{eq:SxSx+SySy} separately. This can be seen by the following observation (see Appendix for a complete proof): for $\forall i$ and $\forall n$, it holds that
\begin{equation}\label{eq:local scar XY}\begin{split}
    \ket*{S_n^{\mr{XY}}}&=\ket{T_{2,2}}_{i,i+1}\otimes\ket*{\Xi^{(2,2)}}+\ket{T_{2,-2}}_{i,i+1}\otimes\ket*{\Xi^{(2,-2)}}\\&+\ket{T_{1,0}}_{i,i+1}\otimes\ket*{\Xi^{(1,0)}}.
    \end{split}
\end{equation}
where $\ket*{\Xi^{(S,M)}}$ is an unnormalized state.
From Eq.\eqref{eq:SxSx+SySy} and Eq.\eqref{eq:local scar XY}, it is trivial that $\ket*{S_n^{\mr{XY}}}$ is annihilated by $S_i^xS_{i+1}^x+S_i^yS_{i+1}^y$. Also, we find
\begin{equation}
    D\sum_i\left(S_i^z\right)^2+h\sum_iS_i^z\ket*{S_n^{\mr{XY}}}=E_n\ket*{S_n^{\mr{XY}}}.
\end{equation}

In summary, the spectrum-generating term in this model is the Zeeman term and the easy-plane anisotropy, which are diagonal in the standard basis, and anisotropic Heisenberg interaction serves as a local annihilator.
%@@@@@@@@@@this should be in Appendix@@@@@@@@@@@@@@@@
\begin{comment}
\subsubsection{Generalization to arbitrary dimensions}
We extend the Hamiltonian Eq.\eqref{eq:one dim XY} to an arbitrary dimension.
\begin{equation}
    H_{\mr{XY}}=J\sum_{\expval{i,j}}\left(S_i^xS_j^x+S_i^yS_j^y\right)+h\sum_iS_i^z+D\sum_i(S_i^z)^2,
\end{equation}
where $\expval{i,j}$ denotes the nearest neighboring sites $i$ and $j$, and we assume PBC. We define the coordinate of a site $i$ as $i\equiv\begin{pmatrix}i_1&\cdots&i_M\end{pmatrix}$ for a $M$ dimensional system. The scar states are also generated by the creation operator $Q_{\mr{XY}}^\dag\equiv\sum_i(-1)^i\left(S_i^+\right)^2$ with $(-1)^i\equiv(-1)^{\sum_{k=1}^Mi_k}$ and by the ferromagnetic state $\ket{\Omega}=\bigotimes_i\ket{-}_i$. We will show $S_i^xS_j^x+S_i^yS_j^y$ annihilates the scar states in the same way as we did in the one dimensional system: it is written as
\begin{equation}\label{eq:SxSx+SySy in higher dimension}
    \begin{split}
        S_i^xS_j^x+S_i^yS_j^y&=2\left(P_{i,j}^{(2,2)}+P_{i,j}^{(2,-2)}+P_{i,j}^{(1,0)}-1\right)\\&+3\left(P_{i,j}^{(2,1)}+P_{i,j}^{(2,0)}+P_{i,j}^{(2,-1)}\right)\\
        &+P_{i,j}^{(1,1)}+P_{i,j}^{(1,-1)}\\+\frac{3}{4}&\left(\ket{T_{2,0}}+\ket{T_{0,0}}\right)\left(\bra{T_{2,0}}+\bra{T_{0,0}}\right)_{i,j}.
    \end{split}
\end{equation}
As is the case with the one dimensional system, the scar states are annihilated by $P_{i,j}^{(2,2)}+P_{i,j}^{(2,-2)}+P_{i,j}^{(1,0)}-1$, and by any other projection operator in Eq.\eqref{eq:SxSx+SySy in higher dimension} separately. In exactly the same manner, one can show that for $\forall i$ and $\forall n$, it holds that
\begin{equation}\begin{split}
    \ket*{S_n^{\mr{XY}}}&=\ket{T_{2,2}}_{i,j}\otimes\ket*{\Xi^{(2,2)}}+\ket{T_{2,-2}}_{i,j}\otimes\ket*{\Xi^{(2,-2)}}\\&+\ket{T_{1,0}}_{i,j}\otimes\ket*{\Xi^{(1,0)}},
    \end{split}
\end{equation}
where the site $j$ is the nearest neighbor of the site $i$ and $\ket*{\Xi^{(S,M)}}$ is an unnormalized state. Thus, $\ket*{S_n^{\mr{XY}}}$ is annihilated by $S^x_iS^x_j+S^y_iS^y_j$. 

In summary, the spectrum-generating term in this model is the Zeeman term and the easy-plane anisotropy, which are diagonal in the standard basis, and anisotropic Heisenberg interaction serves as a local annihilator.
\end{comment}
\subsection{Spin-1/2 domain-wall conserving model}
The domain-wall conserving spin-$1/2$ model~\cite{tos_exact_2} is given by
\begin{equation}\label{eq:DW model}
    H_{\mr{DW}}=\sum_i^N\lambda\left(X_i-Z_{i-1}X_iZ_{i+1}\right)+\Delta Z_i+JZ_iZ_{i+1},
\end{equation}
where $X\equiv\dyad{\uparrow}{\downarrow}+\dyad{\downarrow}{\uparrow}, Z\equiv\dyad{\uparrow}{\uparrow}-\dyad{\downarrow}{\downarrow}$ are the Pauli matrices, and we assume PBC. This model hosts the scar states, which are generated by the creation operator $Q_{\mr{DW}}^\dag\equiv\sum_i(-1)^iP_{i-1}^\downarrow\sigma_i^+P_{i+1}^\downarrow$ with $P^\downarrow\equiv\dyad{\downarrow}$ and $\sigma^+\equiv\dyad{\uparrow}{\downarrow}$ acting on the ferromagnetic state $\ket{\Omega}\equiv\bigotimes_i\ket{\downarrow}_i$. It is shown that the scar state $\ket*{S_n^{\mr{DW}}}\equiv\mc{N}_n^{-1}\left(Q_{\mr{DW}}^\dag\right)^n\ket{\Omega}$ has an energy $E_n=2(\Delta-2J)n+J(N-1)-\Delta N$ and that the first term in Eq.\eqref{eq:DW model} annihilates the scar states~\cite{tos_exact_2}. We will see that the first term consists of local annihilators. It is expressed as
\begin{equation}\begin{split}
    &\sum_i^NX_i-Z_{i-1}X_iZ_{i+1}\\&=2\sum_i^N\left[P_{i-1}^\downarrow X_iP^\uparrow_{i+1}+P^\uparrow_{i-1}X_iP_{i+1}^\downarrow\right],
    \end{split}
\end{equation}
where $P^\uparrow\equiv\dyad{\uparrow}$.
One can show that $P_i^\uparrow X_{i+1}P_{i+2}^\downarrow+P_{i-1}^\downarrow X_iP^\uparrow_{i+1}$ is a local annihilator by the following observation: for $\forall i$ and $\forall n$, $\ket*{S_n^{\mr{DW}}}$ is expressed as 
\begin{equation}\label{eq:local scar DW}
    \begin{split}
        \ket*{S_n^{\mr{DW}}}&=\sum_{\sigma,\sigma'}\ket{\sigma}_{i-1}\ket{\downarrow}_i\ket{\downarrow}_{i+1}\ket{\sigma'}_{i+2}\otimes\ket*{\Xi^0_{\sigma\sigma'}}\\&+\ket{\downarrow}_{i-1}\left(\ket{\uparrow}_i\ket{\downarrow}_{i+1}-\ket{\downarrow}_i\ket{\uparrow}_{i+1}\right)\ket{\downarrow}_{i+2}\otimes\ket*{\Xi^1}\\
        &+\ket{\uparrow}_{i-1}\ket{\downarrow}_i\ket{\uparrow}_{i+1}\ket{\downarrow}_{i+2}\otimes\ket*{\Xi^{2,L}}\\&+\ket{\downarrow}_{i-1}\ket{\uparrow}_i\ket{\downarrow}_{i+1}\ket{\uparrow}_{i+2}\otimes\ket*{\Xi^{2,R}},
    \end{split}
\end{equation}
with $\ket*{\Xi^0_{\sigma\sigma'}}$, $\ket*{\Xi^1}$, and $\ket*{\Xi^{2,L/R}}$ are unnormalized states.  

From Eq.\eqref{eq:local scar DW}, it is trivial that $\ket*{S_n^{\mr{DW}}}$ is annihilated by $P_{i-1}^\downarrow X_iP^\uparrow_{i+1}+P^\uparrow_iX_{i+1}P_{i+2}^\downarrow$. Also one finds
\begin{equation}\begin{split}
    &\sum_i^N\Delta Z_i+JZ_iZ_{i+1}\ket*{S_n^{\mr{DW}}}=E_n\ket*{S_n^{\mr{DW}}}.
    \end{split}
\end{equation}

In summary, the spectrum-generating term in this model is a sum of the Zeeman term and Ising interaction, which are diagonal in the standard spin-$1/2$ basis, and the local annihilator is a spin-flipping term. 

\subsection{The Affleck-Kennedy-Lieb-Tasaki model}
The Affleck-Kennedy-Lieb-Tasaki (AKLT) model is a one-dimensional spin chain. This model contains scar states called ``two-magnon". We will see that the AKLT model allows the same decomposition Eq.~\eqref{eq:basic scheme}, and an annihilator can be local when we enlarge the Hilbert space.
%\subsubsection{Spin-$1$ case}
When each spin has $S=1$, the AKLT model is given as
\begin{equation}
    H_{\mr{AKLT}}=\sum_{i=1}^N\sum_{M=-2}^2P_{i,i+1}^{(2,M)},
\end{equation}
where we assume PBC. The unique ground state of this model is referred to as the valence-bond solid (VBS) state, which we denote $\ket*{\Phi_{\mr{VBS}}}$. The VBS state can be expressed as the matrix product state (MPS), or the Schwinger boson representation. Here, we express the VBS state by fractional spin-$1/2$ representation: any state consisting of two spin-$1/2$s is either the singlet or the triplet, and the triplet has $S=1$. Let $\mc{P}_i:\mb{C}^{2\otimes2}\rightarrow\mb{C}^3$ be a projection operator of two spin-$1/2$s at the site $i$ onto the triplet. Namely, action of $\mc{P}_i$ is defined as 
\begin{equation}\begin{split}
    \mc{P}_i\ket{\uparrow}_{i,\mr{L}}\ket{\uparrow}_{i,\mr{R}}&=\ket{+}_i\\
    \mc{P}_i\ket{\uparrow}_{i,\mr{L}}\ket{\downarrow}_{i,\mr{R}}&=\frac{1}{\sqrt{2}}\ket{0}_i\\
    \mc{P}_i\ket{\downarrow}_{i,\mr{L}}\ket{\uparrow}_{i,\mr{R}}&=\frac{1}{\sqrt{2}}\ket{0}_i\\
    \mc{P}_i\ket{\downarrow}_{i,\mr{L}}\ket{\downarrow}_{i,\mr{R}}&=\ket{-}_i,
    \end{split}
\end{equation}
where the subscripts L and R are introduced to distinguish two spin-$1/2$s at the same site, and $\ket{\pm}_i$ and $\ket{0}_i$ are the standard basis of the spin-$1$ state, satisfying $S_i^z\ket{\pm}_i=\pm\ket{\pm}_i, S_i^z\ket{0}=0$.

With this operator, $\ket{\Phi_{\mr{VBS}}}$ is written as
\begin{equation}
    \ket{\Phi_{\mr{VBS}}}=\left(\bigotimes_{i=1}^N\mc{P}_i\right)\bigotimes_{j=1}^N\ket{\psi_s}_{j,j+1},
\end{equation}
where
\begin{equation}
    \ket{\psi_s}_{j,j+1}\equiv\frac{1}{\sqrt{2}}\left(\ket{\uparrow}_{j,\mr{R}}\ket{\downarrow}_{j+1,\mr{L}}-\ket{\downarrow}_{j,\mr{R}}\ket{\uparrow}_{j+1,\mr{L}}\right).
\end{equation}

Note that for any operator-valued function $f(\bm{S}_i)$, it holds that $f(\bm{S}_i)\mc{P}_i=\mc{P}_if(\bm{S}_{i,\mr{L}}+\bm{S}_{i,\mr{R}})$ as an operator identity. Here $\bm{S}_{i,\mr{L/R}}$ is a spin-$1/2$ operator acting on $\ket{\sigma}_{i,\mr{L/R}}$. Particularly, we can induce a Hamiltonian for a spin-$1/2$
chain from $H_{\mr{AKLT}}$ with the projection:
\begin{equation}
    \begin{split}
        H_{\mr{AKLT}}\left(\bigotimes_{i=1}^N\mc{P}_i\right)&=\left(\bigotimes_{i=1}^N\mc{P}_i\right)\widetilde{H}_{\mr{AKLT}}\\
        &=\left(\bigotimes_{i=1}^N\mc{P}_i\right)\left(\sum_{i=1}^N\sum_{M=-2}^2\widetilde{P}^{(2,M)}_{i,i+1}\right),
    \end{split}
\end{equation}
where $\widetilde{P}_{i,j}^{(S,M)}$ is a projection operator onto the state $\ket*{\widetilde{T}_{S,M}}_{i,j}$ with 4 spin-$1/2$s such that 
\begin{equation}
    \begin{split}
        &\left(\sum_{k=i,i+1}\bm{S}_{k,\mr{L}}+\bm{S}_{k,\mr{R}}\right)^2\ket*{\widetilde{T}_{S,M}}_{i,j}=S(S+1)\ket*{\widetilde{T}_{S,M}}_{i,j}\\
        &S_{i,\mr{L}}^z+S_{i,\mr{R}}+S_{i+1,\mr{L}}^z+S_{i+1,\mr{R}}^z\ket*{\widetilde{T}_{S,M}}_{i,j}=M\ket*{\widetilde{T}_{S,M}}_{i,j}.
    \end{split}
\end{equation}

The scar states of this model, which we denote $\ket*{S_n^{\mr{AKLT}}}$, are generated by the creation operator $Q_{\mr{AKLT}}^\dag\equiv\sum_i(-1)^i(S_i^+)^2$ acting on the VBS state, i.e., $\ket*{S_n^{\mr{AKLT}}}=\mc{N}^{-1}\left(Q^\dag_{\mr{AKLT}}\right)^n\ket*{\Phi_{\mr{VBS}}}$ with a normalization factor $\mc{N}$. One can show the following: for $\forall n$ and $\forall i$, the scar state $\ket*{S_n^{\mr{AKLT}}}$ is expressed as
\begin{equation}\label{eq:aklt scar state}
    \begin{split}
        \ket*{S_n^{\mr{AKLT}}}&=\left(\mc{P}_i\otimes\mc{P}_{i+1}\right)\Big[\ket{\psi_s}_{i,i+1}\otimes\ket*{\Xi^{\sigma\sigma'}}\\+&\ket{\uparrow\uparrow}_i\ket{\uparrow\uparrow}_{i+1}\otimes\ket*{\Xi^{(2,2)}}\\+&\left(\ket{\downarrow\uparrow}_i\ket{\uparrow\uparrow}_{i+1}+\ket{\uparrow\uparrow}_i\ket{\uparrow\downarrow}_{i+1}\right)\otimes\ket*{\Xi^{(2,1)}}\Big]\\&
        \equiv\left(\mc{P}_i\otimes\mc{P}_{i+1}\right)\ket*{\widetilde{S}_n^{\mr{AKLT}}}_{i,i+1},
    \end{split}
\end{equation}
where $\ket{\sigma\sigma'}_i\equiv\ket{\sigma}_{i,\mr{L}}\ket{\sigma'}_{i+1,\mr{R}}$ and $\ket*{\Xi^{\sigma\sigma'}}, \ket*{\Xi^{(2,2)}}$, and $\ket*{\Xi^{(2,1)}}$ are some unnormalized states. From Eq.\eqref{eq:aklt scar state}, one finds that $P_{i,i+1}^{(2,M)}\,\,(M=-2\sim0)$ annihilates $\ket*{S_n^{\mr{AKLT}}}$ and that $\widetilde{P}_{i,i+1}^{(2,2)}+\widetilde{P}_{i,i+1}^{(2,1)}-S_{i,\mr{R}}^z-S_{i+1,\mr{L}}^z$ annihilates $\ket*{\widetilde{S}_n^{\mr{AKLT}}}_{i,i+1}$. Thus, all annihilators are local in spin-$1/2$ representation, but in the original spin-$1$ basis, one of the annihilators becomes non-local as
\begin{equation}\begin{split}
    \left(\bigotimes_{i=1}^N\mc{P}_i\right)\left(\sum_{j=1}^N\widetilde{P}_{j,j+1}^{(2,2)}+\widetilde{P}_{j,j+1}^{(2,1)}-S_{j,\mr{L}}^z-S_{j+1,\mr{R}}^z\right)\\
    =\sum_j\left(P_{j,j+1}^{(2,2)}+P_{j,j+1}^{(2,1)}-S_j^z\right)\left(\bigotimes_{i=1}^N\mc{P}_i\right).
    \end{split}
\end{equation}
It is trivial to see $\sum_iS_i^z\ket*{S_n^{\mr{AKLT}}}=2n\ket*{S_n^{\mr{AKLT}}}$.

In summary, the spectrum generating term of the AKLT model is the Zeeman term $\sum_iS_i^z$, and the annihilators are either $P_{i,i+1}^{(2,M)}\,\,(M=-2\sim0)$ or $\sum_i(P_{i,i+1}^{(2,2)}+P_{i,i+1}^{(2,1)}-S_i^z)$. The latter annihilator can be expressed as a sum of local terms, each of which annihilates the (induced) scar states in the spin-$1/2$ representation.   

% this can be in appendix@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@
\begin{comment}
\subsubsection{Spin-$S$ case}
The idea of fractional spin-$1/2$ can be used for the scar states in the general spin-$S$ AKLT model, which is defined as
\begin{equation}
    H^S_{\mr{AKLT}}=\sum_{i=1}^N\sum_{J=S+1}^{2S}\sum_{M=-J}^JP_{i,i+1}^{(J,M)}.
\end{equation}
We can define a similar projection operator for this case. Let $\mc{P}_i^S:\mb{C}^{2\otimes2S}\rightarrow\mc{C}^{2S+1}$ be the projection operator of $2S$ spin-$1/2$ at the site $i$ onto states with total spin $S$. With this operator, the ground state of this model, which we denote the spin-$S$ VBS state $\ket*{\Phi^S_{\mr{VBS}}}$, is written as
\begin{equation}
    \ket{\Phi_{\mr{VBS}}^S}=\left(\bigotimes_{i=1}^N\mc{P}_i\right)\bigotimes_{j=1}^N\ket{\psi^S_s}_{j,j+1},
\end{equation}
where 
\begin{equation}\begin{split}
    \ket{\psi^S_s}_{j,j+1}\equiv\bigotimes_{l=1}^S\frac{1}{\sqrt{2}}&\left(\ket{\uparrow}_{(j,l),\mr{R}}\ket{\downarrow}_{(j+1,l),\mr{L}}\right.\\&\left.-\ket{\downarrow}_{(j,l),\mr{R}}\ket{\uparrow}_{(j+1,l),\mr{L}}\right),
    \end{split}
\end{equation}
where we introduce the additional index $l$ to distinguish $S$ spin-$1/2$s at L or R at the site $i$.

The scar states, denoted as $\ket*{S_n^{S\mr{-AKLT}}}$, are generated by the creation operator $Q^\dag_{S\mr{-AKLT}}\equiv\sum_i(-1)^i(S_i^+)^{2S}$ acting on the spin-$S$ VBS state, i.e., $\ket*{S_n^{S\mr{-AKLT}}}=\mc{N}^{-1}\left(Q^\dag_{S\mr{-AKLT}}\right)^2\ket*{\Phi_{\mr{VBS}}^S}$ with a normalization factor $\mc{N}$. One can show that the scar states are annihilated by $P_{i,i+1}^{(J,M)}\,\,(\forall J,\,\, M\leq S)$ for $\forall i$ and by $\sum_i(\sum_{J=S+1}^{2S}\sum_{M=S}^JP_{i,i+1}^{(J,M)})-\frac{1}{S}S_i^z$. The latter annihilator can be expressed as a sum of local annihilators (see Appendix for a detailed derivation).  
\end{comment}
%@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@

==> files_not_used/scar_state_old.tex <==
%\label{magnon}
\textit{The scar states--.} 
%In this section, we construct the scar states approximately. In what follows, we only consider PBC, i.e., $H_{\mr{PBC}}$.

%Numerical results show that the scar states, denoted as $\ket{\mc{S}_n}$, have energies almost proportional to $1.33$, i.e., $H_{\mr{PBC}}\ket{\mc{S}_n}=E_n\ket{\mc{S}_n}$ with $E_n\cong1.33n$ (see Fig.[FIG]). We first consider $\ket{\mc{S}_1}$, then extend our argument to general states $\ket{\mc{S}_n}$.

\subsection{\label{subsec:|S1>}Approximation for $\ket{\mc{S}_1}$}
\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{aklt_x_pol.pdf}
    \caption{A typical configuration of the approximated scar states. The dimer at some bond is broken and a pair of fractional spins is polarized.}
    \label{fig:aklt_x_pol}
\end{figure}
As seen in Sec.\ref{subsec:exact eigenstates for OBC}, the Zeeman term $\sqrt{2}\sum_bS_b^x$ is responsible for the energies of the four exact eigenstates for $H_{\mr{OBC}}$, and those states are understood as the polarization of edge spin-$1/2$s. Though this is not directly applicable to $H_{\mr{PBC}}$, it is still natural to guess that the Zeeman term is also responsible for the equidistant energies of the scar states, noting that the ``magnetic field" $\sqrt{2}\cong1.41$ in the Zeeman term is close to the observed energy spacing $1.33$. Motivated by this observation, we consider the following trial wave function $\ket*{S_1^{\mr{PXP}}}$:
\begin{equation}
    \ket*{S^{\mr{PXP}}_1}\equiv\sum_{b=1}^N(-1)^bP_{\mr{Ryd}}\ket*{M_b},
\end{equation}
where  
\begin{equation}\begin{split}
    \ket*{M_b}\equiv&\left(\bigotimes_{b'=1}^N\mc{P}_{b'}\right)\bigotimes_{b''\not=b}\ket*{\psi_s}_{b'',b''+1}\otimes\ket*{\rightarrow}_{b,\mr{R}}\ket*{\rightarrow}_{b+1,\mr{L}}\\
    P_{\mr{Ryd}}&\equiv\prod_n\left(1-P_{2n-1,2n}^{(2,2)}\right)\left(1-P_{2n,2n+1}^{(2,-2)}\right)
    \end{split}
\end{equation}
Namely, the dimer at the bond between $b$ and $b+1$ is broken as those spin-$1/2$s are polarized in $+x$-direction in $\ket*{M_b}$.

We show $\ket*{S^{\mr{PXP}}_1}$ is a good approximation to the scar state $\ket{\mc{S}_1}$. One finds
\begin{equation}\label{eq:H|S1>=E|S1>+|N>}
    H_{\mr{PBC}}\ket{S^{\mr{PXP}}_1}=\sqrt{2}\ket{S^{\mr{PXP}}_1}-\frac{\sqrt{2}}{4}\ket{N_{\mr{odd}}}+\frac{\sqrt{2}}{4}\ket{N_{\mr{even}}},
\end{equation}
where
\begin{widetext}
\begin{equation}
    \begin{split}
        \ket{N_{\mr{odd}}}&=\sum_n\left(\bigotimes_{b\not=2n-1,2n}\mc{P}_b\right)\bigotimes_{b'\not=2n-2\sim2n}\ket*{\psi_s}_{b',b'+1}\otimes\ket{\downarrow}_{2n-2,\mr{R}}\ket{T_{2,1}}_{2n-1,2n}\ket{\downarrow}_{2n+1,\mr{L}}\\
        \ket{N_{\mr{even}}}&=\sum_n\left(\bigotimes_{b\not=2n,2n+1}\ms{S}_b\right)\bigotimes_{b'\not=2n-1\sim2n+1}\ket*{\psi_s}_{b',b'+1}\otimes\ket{\uparrow}_{2n-2,\mr{R}}\ket{T_{2,-1}}_{2n,2n+1}\ket{\uparrow}_{2n+1,\mr{L}}.
    \end{split}
\end{equation}
\end{widetext}

\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{m_odd.pdf}
    \caption{Caption}
    \label{fig:m_odd}
\end{figure}
We further decompose $(-\ket{N_{\mr{odd}}}+\ket{N_{\mr{even}}})/4$ into a component parallel to $\ket*{S^{\mr{PXP}}_1}$ and a component perpendicular to it, denoted as $\ket*{S_1^\perp}$. From a straightforward calculation (see Appendix for a detail of derivation), one obtains the energy correction:
\begin{equation}\begin{split}
    \delta(N)\equiv\frac{1}{4}\bra{S_1}\left(-\ket{N_{\mr{odd}}}+\ket{N_{\mr{even}}}\right)\rightarrow-\frac{1}{14},
    \end{split}
\end{equation}
as $N\rightarrow\infty$.

Therefore, one can re-write Eq.~\eqref{eq:H|S1>=E|S1>+|N>} as
\begin{equation}
    H_{\mr{PBC}}\ket{S_1}=\sqrt{2}\left(1-\delta(N)\right)\ket{S_1}+\sqrt{2}\ket{S_1^\perp}.
\end{equation}
An approximate energy of $\ket{S_1}$ is about $\sqrt{2}\times13/14\cong1.31$ for a sufficiently large $N$, which is close to the observed energy $1.33$.

We can also show that a squared norm of $\ket{S_1^\perp}$ remains relatively small:
\begin{equation}
    \frac{\braket*{S_1^\perp}}{\braket{S_1}}=\frac{11}{3\times14^2}\cong1.87\times10^{-2}.
\end{equation}

In fact, we confirm by numerics that $|\braket{S_1}{\mc{S}_1}|^2/\sqrt{\braket{S_1}}\cong0.6206$ 
for $N=10$, which implies that $\ket{S_1}$ is a good approximation. 

Physically, the state $\ket{S_1}$ is understood as a magnon-like excitation of a pair of fractional spin-$1/2$s in $+x$-direction with a momentum $\pi$ and the Zeeman term is almost responsible for the energy, while the other terms give a correction.
\subsection{\label{subsec:|S_n>}Approximation for $\ket{\mc{S}_n}$}
We generalize our consideration on $\ket{\mc{S}_1}$ to other scar states $\ket{\mc{S}_n}$. A key idea is to regard the scar states as $n$ magnon excitations, as seen in Sec.~\ref{subsec:|S1>}. In order to create such excitations at bond between $b$ and $b+1$, we need to break the singlet there and make them polarize in the $x$-direction. This is done by acting on the singlet $(\ket{\uparrow}_{b,\mr{R}}\ket{\downarrow}_{b+1,\mr{L}}-\ket{\downarrow}_{b,\mr{R}}\ket{\uparrow}_{b+1,\mr{L}})/\sqrt{2}$ an operator $S_{b,\mr{R}}^{x+}-S_{b+1,\mr{L}}^{x+}$ with $S_{b,\mr{L/R}}^{x\pm}\equiv S_{b,\mr{L/R}}^y\pm iS_{b,\mr{L/R}}^z$. The momentum $\pi$ implies that we should consider $\sum_b(-1)^b\left(S_{b,\mr{R}}^{x+}-S_{b+1,\mr{L}}^{x+}\right)$. Together with the Rydberg constraint, we construct our approximate wave function $\ket*{S_n^{\mr{PXP}}}$ for $\ket{\mc{S}_n}$: for $n>0$, it is defined as 
\begin{equation}\label{eq:|S_n>}\begin{split}
    \ket*{S^{\mr{PXP}}_n}\equiv P_{\mr{Ryd}}\left(\sum_b(-1)^b\left(S_b^y+iS_b^z\right)\right)^n\ket*{\Phi_{\mr{VBS}}},
\end{split}
\end{equation}
and for $n<0$, it is
\begin{equation}
    \ket*{S^{\mr{PXP}}_n}\equiv P_{\mr{Ryd}}\left(\sum_b(-1)^b\left(S_b^y-iS_b^z\right)\right)^{|n|}\ket{\Phi_{\mr{VBS}}}.
\end{equation}
Fig.~\ref{fig:magnon_results} shows overlap between $\ket*{S_n^{\mr{PXP}}}$ and $\ket{\mc{S}_n}$ which is numerically determined for $1\leq n\leq 10$ and for $N=10$.  
\begin{figure}
    \centering
    \includegraphics[width=.48\textwidth]{magnon_results.pdf}
    \caption{The squared overlap between our approximation and the corresponding exact scar state $|\braket{S_n}{\mc{S}_n}|^2/\braket{S_n}$ for $N=10$.}% (blue dots) and $|\braket{S'_n}{\mc{S}_n}|^2/\braket{S'_n}$ (orange dots) for $N=10$.}
    \label{fig:magnon_results}
\end{figure}
The overlap is more than $80\%$ except for $n=1$, implying a validity of our approximation. %I should try P_ryd(sum Sy+iSz)^n!! 
This trial wave function can be re-written by the creation operator $Q_{\mr{PXP}}^\dag\equiv\sum_b(-1)^b(S_b^y+iS_b^z)$ as 
\begin{equation}\label{eq:Qpxp|VBS>}
    \ket*{S_n^{\mr{PXP}}}=
    \begin{dcases}
    P_{\mr{Ryd}}\left(Q_{\mr{PXP}}^\dag\right)^n\ket{\Phi_{\mr{VBS}}}\quad(n>0)\\
    P_{\mr{Ryd}}\left(Q_{\mr{PXP}}\right)^{|n|}\ket{\Phi_{\mr{VBS}}}\quad(n<0)
    \end{dcases}.
\end{equation}
An important difference between this wave function and the scar states in other models discussed in Sec.~[SEC] is that we need to enlarge the Hilbert space by ignoring the Rydberg constraint when we consider the scar states in the PXP model. Indeed, $P_{\mr{Ryd}}Q_{\mr{PXP}}^\dag P_{\mr{Ryd}}$ is neither equivalent to Eq.~\eqref{eq:Qpxp|VBS>} as $P_{\mr{Ryd}}(Q_{\mr{PXP}}^\dag)^n\not=(P_{\mr{Ryd}}Q_{\mr{PXP}}^\dag P_{\mr{Ryd}})^n$, nor a good creation operator, as it produces states with small overlap with the scar states. 

Note that $\ket*{\mc{S}_N}$ is the highest excited state, and Eq.~\eqref{eq:|S_n>} shows that it is well-approximated by the fully $x$-polarized (FP) state, projected onto the constrained subspace, i.e., $\ket{S_N^{\mr{PXP}}}=P_{\mr{Ryd}}\ket*{\Phi_{\mr{FP}}^+}$ where %we find that this state is very well-approximated by the following fully polarized (FP) state in the constrained subspace, i.e., $P_{\mr{Ryd}}\ket*{\Phi_{\mr{FP}}^+}$, where
\begin{equation}
    \ket*{\Phi_{\mr{FP}}^+}\equiv\bigotimes_{b=1}^N\left(\frac{1}{2}\ket{+}+\frac{1}{\sqrt{2}}\ket{0}+\frac{1}{2}\ket{-}\right)_b.
\end{equation}
A state $\frac{1}{2}\ket{+}+\frac{1}{\sqrt{2}}\ket{0}+\frac{1}{2}\ket{-}$ is the eigenstate of $S^x$ with eigenvalue $+1$. Therefore, $\ket*{\Phi_{\mr{FP}}^+}$ is interpreted as a state with all spin-$1$s polarized in $+x$-direction, which maximizes the Zeeman term.

\subsection{Approximate wave function based on the FP state}
We can construct another approximate wave function $\ket*{S'^{\mr{PXP}}_n}$ for $\ket{\mc{S}_n}$ by exciting $n$ magnons on top of the FP state. It is defined as
\begin{equation}
    \ket{S'^{\mr{PXP}}_n}=\begin{dcases}
    \left(Q_{\mr{PXP}}\right)^{N-n}\ket{\Phi_{\mr{FP}}^+}\quad(n>0)\\
    \left(Q^\dag_{\mr{PXP}}\right)^{n-N}\ket{\Phi_{\mr{FP}}^-}\quad(n<0)
    \end{dcases},
\end{equation}
where 
\begin{equation}
    \ket{\Phi_{\mr{FP}}^-}\equiv\bigotimes_{b=1}^N\left(\frac{1}{2}\ket{+}-\frac{1}{\sqrt{2}}\ket{0}+\frac{1}{2}\ket{-}\right)_b.
\end{equation}
Note that $\frac{1}{2}\ket{+}-\frac{1}{\sqrt{2}}\ket{0}+\frac{1}{2}\ket{-}$ is the eigenstate of $S^x$ with eigenvalue $-1$.

Fig.~[FIG] shows squared overlap between $\ket*{S'^{\mr{PXP}}_n}$ and $\ket{\mc{S}_n}$. Although $\ket*{S'^{\mr{PXP}}_n}$ is slightly worse approximation for $\ket{\mc{S}_n}$ than $\ket*{S^{\mr{PXP}}_n}$ particularly when $n$ is large, $\ket{S'^{\mr{PXP}}_n}$ is also a good approximation.


In summary, we can obtain the scar states approximately by regarding them as magnons. Numerics on the overlap between our approximations ($\ket*{S_n^{\mr{PXP}}}$ and $\ket*{S'^{\mr{PXP}}_n}$) and the corresponding exact scar states $\ket{\mc{S}_n}$ supports our idea. Particularly, the ground state and the the highest excited state are understood as the FP states where all spins are polarized in $\pm x$-direction. Note that the almost equidistant energies are due to the Zeeman term.

\subsection{Perturbations and a possible mechanism of scar states}
It is known that certain perturbations to $H_{\mr{PBC}}$ yields longer revivals. We consider two types of perturbations and numerically show that our trial wave function $\ket{S'^{\mr{PXP}}_n}$ becomes a very accurate approximation for the scar state. This observation suggests that we can understand the modified PXP model in the form Eq.~\eqref{eq:basic scheme}, namely a spectrum-generating term and annihilators.
\subsubsection{Perturbations from the emergent $SU(2)$ algebra approach}
In Ref.~[REF], the following perturbation is considered: in the original spin-$1/2$ basis, it is
\begin{equation}
    \delta_RH=-\sum_{d=2}^Rh_d\sum_{i=1}^{2N}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}\left(Z_{i-d}+Z_{i+d}\right).
\end{equation}
The coefficient $h_d$ is set to be $h_d=h_0(\phi^{d-1}-\phi^{1-d})^{-2}$ with the golden ratio $\phi=(1+\sqrt{5})/2$ and $h_0\cong0.05$. Fig.~[FIG] shows overlap between numerically eigenstates of $H_{\mr{PBC}}+\delta_RH$ and the N\'eel state for $R=N=10$. This figure suggests to identify a set of states in the outermost layer with the scar states $\ket{\mc{S}_n}$. The scar states have a more dominant contribution to the N\'eel state, which yields longer revivals.  

We try our approximate wave functions $\ket*{S_n^{\mr{PXP}}}$ and $\ket*{S'^{\mr{PXP}}_n}$. Fig.~[FIG] shows squared overlap between the trial wave functions and the scar states for $N=R=10$. The ansatz build on the FP state $\ket*{S'^{\mr{PXP}}_n}$ becomes much better ($\sim96\%$ match) while the ansatz build on the VBS state $\ket{S_n^{\mr{PXP}}}$ becomes worse. Note that the energy spacing of the tower of states becomes around $1.29$. This suggests that the modified Hamiltonian essentially describes the precession of a large spin around a field $1.29\bm{e}_x$, whereby the state is projected to the constrained subspace. 
\subsubsection{Perturbations from the broken Lie algebra approach}
In Ref.~[REF], perturbations are systematically constructed, motivated by the idea presented in Ref.~[REF]. The process of generating perturbations takes the following steps: first, split the Hamiltonian into a spin ``raising" and a ``lowering" part, i.e., $H_{\mr{PBC}}=H^++H^-$, and define  ``$z$-component" by the commutator of $H^+$ and $H^-$, i.e., $H^z=[H^+, H^-]$. We also calculate the commutator of $H^z$ and $H^\pm$, resulting in $[H^z, H^\pm]=\pm2H^\pm+\delta_\pm H$ with a remaining operator $\delta_\pm H$. Now we regard $\delta_\pm H$ as a correction to $H^\pm$, and redefine the ladder operator as $H^\pm\rightarrow H^\pm+g\delta_\pm H$ with some coefficient $g$ which will be determined later. This modification yields the modification of the Hamiltonian as $H_{\mr{PXP}}\rightarrow H_{\mr{PXP}}+g(\delta_+H+\delta_-H)$. $g$ is determined such that the fidelity of a targeted initial state such as $\ket{\mb{Z}_2}$ after one period of revival should be maximized. We can repeat this procedure to obtain further perturbations.


To maximize the duration of revivals from $\ket{\mb{Z}_2}$, the following perturbations were considered in Ref.~[REF]: $\delta H=\sum_{\lambda=1}^9g_\lambda H_\lambda$, where
\begin{equation}
    \begin{split}
        H_1&=\sum_{i=1}^{2N}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}\left(P^\downarrow_{i-2}+P^\downarrow_{i+2}\right)\\
        H_2&=\sum_{i=1}^{2N}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}\left(P^\downarrow_{i-3}Z_{i-2}+Z_{i+2}P^\downarrow_{i+3}\right)\\
        H_3&=\sum_{i=1}^{2N}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}\left(P^\downarrow_{i-3}P^\downarrow_{i-2}+P^\downarrow_{i+2}P^\downarrow_{i+3}\right)\\
        H_4&=\sum_{i=1}^{2N}P^\downarrow_{i-2}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}P^\downarrow_{i+2}\\
        H_5&=\sum_{i=1}^{2N}P^\downarrow_{i-1}X_iP^\downarrow_{i+2}\left(P^\downarrow_{i-2}Z_{i+2}P^\downarrow_{i+3}+P^\downarrow_{i-3}Z_{i-2}P^\downarrow_{i+2}\right)\\
        H_6&=\sum_{i=1}^{2N}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}\left(Z_{i+2}P^\downarrow_{i+3}P^\downarrow_{i+4}+P^\downarrow_{i-4}P^\downarrow_{i-3}Z_{i-2}\right)\\
        H_7&=\sum_{i=1}^{2N}P^\downarrow_{i-2}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}P^\downarrow_{i+2}\left(P^\downarrow_{i-3}+P^\downarrow_{i+3}\right)\\
        H_8&=\sum_{i=1}^{2N}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}\left(P^\downarrow_{i-3}P^\downarrow_{i-2}P^\downarrow_{i+2}+P^\downarrow_{i-2}P^\downarrow_{i+2}P^\downarrow_{i+3}\right)\\
        H_9&=\sum_{i=1}^{2N}P^\downarrow_{i-4}P^\downarrow_{i-3}Z_{i-2}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}P^\downarrow_{i+2}\\
        &+\sum_{i=1}^{2N}P^\downarrow_{i-2}P^\downarrow_{i-1}X_iP^\downarrow_{i+1}Z_{i+2}P^\downarrow_{i+3}P^\downarrow_{i+4}.
    \end{split}
\end{equation}
We take the coupling constants $g_\lambda$ as the optimal values given in Ref.[REF].  
\begin{figure}
    \centering
    \includegraphics[width=.48\textwidth]{overlap_perturb.pdf}
    \caption{Overlap between the N\'{e}el state and eigenstates for the perturbed Hamiltonian.}
    \label{fig:overlap_perturb}
\end{figure}
Overlap between eigenstates of $H_{\mr{PBC}}+\delta_{\mr{Lie}}H$ and the N\'eel state is shown in Fig.~[FIG]. This figure suggests to identify a set of states in the outermost layer with scar states $\ket{\mc{S}_n}$, and they have a more dominant contribution to the N\'eel state, which is similar to $H_{\mr{PBC}}+\delta_RH$.    

We try our approximate wave functions $\ket*{S^{\mr{PXP}}_n}$ and $\ket*{S'^{\mr{PXP}}_n}$. Fig.~[FIG] shows squared overlap between our approximations and the scar state for $N=10$. Similar to $\delta_RH$, it shows that the ansatz built upon the FP state $\ket*{S'^{\mr{PXP}}_n}$ becomes much better, while the other ansatz built upon the VBS is worse. The energy spacing of the tower of states is very close to $\sqrt{2}$, which implies that the modified Hamiltonian essentially describes the precession of a large spin around a field $\sqrt{2}\bm{e}_x$, whereby the state is projected to the constrained subspace.  
%H_PXP=S^x+else?
%\subsection{Creation Operator\label{subsubsec:creation_pbc}}
%We define the following 3-local operator $Q^\dagger(k)$ as a candidate for a creation operator.
%\begin{equation}\label{eq:creation_pbc}
	%Q^\dagger(k)=\sum_je^{ikj}P_{j-1}\left(Z_j-i\sqrt{\frac{2+\cos k}{2}}Y_j\right)P_{j+1},
%\end{equation} 
%where $Y=-i\dyad{\uparrow}{\downarrow}+i\dyad{\downarrow}{\uparrow}$ and $Z=\dyad{\uparrow}{\uparrow}-\dyad{\downarrow}{\downarrow}$. This operator satisfies the similar commutation relation to Eq.~\eqref{eq:relation}:
%\begin{equation}\label{eq:commutation}
    %\left[H, Q^\dag(k)\right]=\sqrt{2(2+\cos k)}Q^\dag(k)+A(k),
%\end{equation}
%where 
%\begin{equation}\label{eq:remainder}\begin{split}
    %A(k)&=\frac{i}{2}\sum_je^{ikj}P_{j-1}Y_jP_{j+1}\left(e^{-ik}Z_{j-2}+e^{ik}Z_{j+2}\right)\\
    %&+\frac{1}{2}\sqrt{\frac{2+\cos k}{2}}\left(1+e^{-ik}\right)\sum_je^{ikj}P_{j-2}\\
    %&\times\left(X_{j-1}X_j+Y_{j-1}Y_j\right)P_{j+1}.
%\end{split}
%\end{equation}
%Note that {\it any} operator satisfies Eq.~\eqref{eq:relation} by properly defining $A$. However, we choose the coefficient $\sqrt{(2+\cos k)/2}$ in Eq.~\eqref{eq:creation_pbc} so that $A(k)$ does not contain 3-local operators.

%Eq.~\eqref{eq:commutation} is understood as follows. The first term implies that the dispersion of ``quasiparticle" is $\omega(k)=\sqrt{2(2+\cos k)}$. $A(k)$ might preclude the possibility of a closed algebra, which makes states generated by $Q^\dag(k)$ not exact and equidistant. We expect the influence of $A(k)$ is minimized by $k=\pi$, as the last term in Eq.~\eqref{eq:remainder} vanishes. Thus we consider $Q^\dagger(\pi)$ as the creation operator. 

%We can obtain states by acting $Q^\dag(\pi)(\text{or }Q(\pi))$ on $\ket{\psi_{\rm{BCS}}}$ with a spacing expected to be around $\sqrt{2}$, which is close to the result from numerics ($\sim1.33$). Moreover, energy $\sqrt{2}$ is also found in the exact excited states in the open boundary condition \cite{qmbs_aklt_vp}. 

%\subsection{Quality of the Creation Operator}
%Our creation operator $Q^\dag(\pi)$ generates an approximate tower of states $\ket{n}$ on top of the zero energy scarred state $\ket{\psi_{\rm{BCS}}}$ as follows: 
%\begin{equation}\label{eq:approximate tos}
    %\ket{n}=\begin{dcases}\frac{1}{\mathcal{N}_n}\left(Q^\dag(\pi)\right)^n\ket{\psi_{\rm{BCS}}}&\,\,(n>0)\\
    %\ket{\psi_{\rm{BCS}}}&\,\,(n=0)\\
    %\frac{1}{\mathcal{N}_n}\left(Q(\pi)\right)^{|n|}\ket{\psi_{\rm{BCS}}}&\,\,(n<0)
    %\end{dcases},
%\end{equation}
%where $\mathcal{N}_n$ is a normalization factor. 
%We first need to see if the state $\ket{n}$ is a well-approximated eigenstate. %To do so, we study $\gamma_n$ in (\ref{gamma_n}). For our creation and annihilation operators $Q^\dagger(\pi), Q(\pi)$, $\gamma_n$ is defined as follows:  
%\begin{equation}\label{eq:gamma}\begin{split}
	%\gamma_n&=\begin{dcases}\frac{\left\|A(\pi)\ket{n}\right\|}{\sqrt{2}\left\|Q^\dagger(\pi)\ket{n}\right\|}&\,\,(n\geq0)\\
	%\frac{\left\|A(\pi)\ket{n}\right\|}{\sqrt{2}\left\|Q(\pi)\ket{n}\right\|}&\,\,(n<0)
	%\end{dcases}
	%\end{split}
%\end{equation}  
%Since $\gamma_n$ is connected to $\gamma_{-n}$ by particle-hole symmetry $\prod_iZ_i$, it suffices to look at $\gamma_n$ for $n\geq0$ only.
%\begin{figure}
    %\centering
    %\includegraphics[width=0.48\textwidth]{overlap_diagonal.pdf}
    %\caption{Overlap between the approximate tower of states defined in Eq.~\eqref{eq:approximate tos} and the exact tower of states. We choose the optimized BCS ansatz as a reference state.}
    %\label{fig:overlaps_diagonal}
%\end{figure}
%We find our approximation describes the tower of states very accurately for small $n$. As shown in Fig.~\ref{fig:overlaps_diagonal}, our approximation becomes less accurate when $|n|$ is large, as expected. We note that the ground state and the highest excited state, living at the edges of the spectrum in Fig.\ref{fig:pbc_z2overlap_n_14}, are not captured by $Q^\dag(\pi)$ and $Q(\pi)$. We also find that $\ket{n}$ with large $n$, though it is a less accurate approximation of the corresponding exact scarred state $\ket{\psi_n}$, is well described by a superposition of the exact scarred states (Fig.\ref{fig:weight}).%However, this does not mean $Q^\dag(\pi)$ cannot capture scarred states with large $n$ at all, since the weight $\mathcal{W}(n)=\sum_{m=-9}^{9}\left|\bra{\psi_m}\ket{n}\right|^2$ for $N=20$ suggests that even for large $n$, $\ket{n}$ is regarded as a superposition of exact scarred states (Fig.~\ref{fig:weight}). Therefore $\ket{n}$ with a large $n$ still carries some information of the scarred states.
%\begin{figure}
    %\centering
    %\includegraphics[width=.48\textwidth]{weight.pdf}
    %\caption{Weight $\mathcal{W}(n)=\sum_{m=-9}^9\left|\bra{\psi_m}\ket{n}\right|^2$ of each approximate scarred state for $N=20$.}
    %\label{fig:weight}
    %\includegraphics[width=.48\textwidth]{overlaps_scarred_editted.eps}
    %\caption{Overlaps of approximate scarred states with exact scarred states $\left|\bra{\psi_n}\ket{n}\right|^2$ when the system size $N$ is varied.}
%\end{figure}

%We also see how much $A(\pi)$ affects our scarred states, which is quantified by $\gamma_n$ in Eq.~\eqref{eq:gamma_n}.
%\begin{figure}[H]
    %\centering
    %\includegraphics[width=0.48\textwidth]{gammas.pdf}
    %\caption{$\gamma_n$ for a small $n$ as the system size is varied.}
    %\label{fig:gamma_n}
%\end{figure}
%Figure \ref{fig:gamma_n} implies that at least for a small $n$, a contribution of $A(\pi)$ does not become dominant even in the thermodynamic limit.
%\begin{comment}
%\begin{figure}
	%\centering
	%\includegraphics[width=.48\textwidth]{gamma_n_exact_2.eps}
	%\caption{\label{fig:gamma_exact}$\gamma_n$ defined in (\ref{eq:gamma}) for $N=4\sim20$. Extrapolation lines show that at the thermodynamic limit $N\rightarrow\infty$, $\gamma_0\rightarrow1.046\times10^{-1},$ $\gamma_1\rightarrow9.582\times10^{-2},$ and $\gamma_2\rightarrow2.121\times10^{-2}$. These lines are based on data points from $N=10$ to $N=20$.}
%\end{figure}
%Figure \ref{fig:gamma_exact} implies that for $N\rightarrow\infty$ the remaining term $A(\pi)$ does not preclude our approximate SGA $\left[H, Q^\dagger(\pi)\right]\sim \sqrt{2}Q^\dagger(\pi)$.
  
%We also study overlap between $n$th exact scarred states $\ket{\epsilon_n}$ with our approximate scarred states $\ket{n}$ as shown in Fig.\ref{fig:overlap_eig_from_ed}.   
%$\ket{n}$ has a very high overlap with the corresponding exact scarred state $\ket{\epsilon_n}$, which supports the validity of our approximate SGA. 
%\begin{figure}
	%\centering
	%\includegraphics[width=.48\textwidth]{overlaps_from_ed_n_20.eps}
	%\caption{\label{fig:overlap_eig_from_ed}Overlap between the exact scarred state $\ket{\epsilon_n}$ (blue dots) or the $\mathbb{Z}_2$ state (red x) and the approximate scarred state $\ket{n}$ generated by $Q^\dagger(\pi)$ or $Q(\pi)$ for $N=20$.}
	%\includegraphics[width=.48\textwidth]{energy_expec_exact.eps}
	%\caption{\label{fig:energy_expec_exact}Energy expectation values $\bra{n}H\ket{n}$ for $N=20$.}
%\end{figure}
%Figure \ref{fig:energy_expec_exact} shows an almost equidistant energy expectation value $\bra{n}H\ket{n}$ for a small $n$. As $n$ gets larger a deviation from the equidistant expectation values become significant. However, this does not invalidate our SGA since $\ket{n}$ is almost a superposition of exact scarred eigenstates. For example, we find $\left|\braket{\epsilon_7|7}\right|^2\sim0.42$ and $\left|\braket{\epsilon_3|7}\right|^2\sim0.30$ (data not shown).   

%We note that our approach is fundamentally different from ``magnon condensation" \cite{magnon_condensation} though both look very similar. The biggest difference is that from our approach we can directly obtain approximate scarred states by applying the creation operator while the method discussed in Ref.\cite{magnon_condensation} suggests a way to restrict the Hilbert space, which means the existence of almost equidistant energies is not understood intuitively.  
%\subsection{\label{subsec:E=0}$E=0$ scarred state}
%Our method depends on the scarred eigenstate with zero energy. On the other hand, it is not always possible to obtain such a state due to a massive degeneracy at $E=0$. Actually, the supplementary material in Ref.\cite{Turner2018} and Ref.\cite{turner_tower} do not capture the zero energy scarred state. In this section we show that it is possible to obtain an approximate zero energy scarred state from adjacent scarred states. 

%We start from the following observation. We define the following state $\ket{\tilde{0}}$
%\begin{equation}\label{eq:zero_state}\begin{split}
	%\ket{\tilde{0}}&=\beta\left(Q(\pi)\ket{\epsilon}-(-1)^{N/2}Q^\dagger(\pi)\ket{-\epsilon}\right)\\
	%&=\beta\left(1-(-1)^{N/2}\mathcal{C}\right)Q(\pi)\ket{\epsilon},
%\end{split}
%\end{equation}  
%where $\beta$ is a normalization factor and $\ket{\pm\epsilon}$ is an adjacent scarred state with $E\cong\pm1.33$. Since $\ket{\tilde{0}}$ is particle-hole symmetric, an energy expectation value $\bra{\tilde{0}}H\ket{\tilde{0}}$ must be zero.

%We find $\left|\braket{\tilde{0}|\mathbb{Z}_2}\right|^2\cong0.164$ for $N=20$, which is anomalously high. We confirm that $\ket{\tilde{0}}$ has a high overlap with $\mathbb{Z}_2$ state for $N=6\sim20$. We also study an overlap between $\ket{\tilde{0}}$ and eigenstates as shown in Fig.\ref{fig:nearly_zero_n_14}, which shows contribution is mostly from $\ket{0}$ and finds $\left|\braket{0|\tilde{0}}\right|^2\cong8.720\times10^{-1}$ for $N=20$. This is also confirmed for $N=6\sim20$.
%\begin{figure}
	%\centering
	%\includegraphics[width=0.48\textwidth]{nearly_zero_n_20.eps}
	%\caption{\label{fig:nearly_zero_n_14}Overlap between $\ket{\tilde{0}}$ and eigenstates for $N=20$.}
%\end{figure}  

%We can construct the scar subspace approximately by applying $Q^\dagger(\pi)$ or $Q(\pi)$ on $\ket{\tilde{0}}$.
%\begin{equation}
	%\ket{n}\equiv\begin{dcases}
		%\beta_n\left(Q^\dagger(\pi)\right)^n\ket{\tilde{0}}&\quad(n>0)\\
		%\ket{\tilde{0}}&\quad(n=0)\\
		%\beta_n\left(Q(\pi)\right)^{|n|}\ket{\tilde{0}}&\quad(n<0)
	%\end{dcases},
%\end{equation}
%with a normalization factor $\beta_n$. 

%\subsection{the Approximate Scar Subspace Using MPS}
%Following the argument in Sec.\ref{subsec:E=0}, we can construct the subspace $\mathcal{V}$ approximately based on MPS ansatz discussed in Ref.\cite{qmbs_aklt_vp}. Approximate scarred states $\ket{\Xi_\pm}$ for $\ket{\epsilon_\pm}$ are constructed as MPS using single mode approximation (SMA) on top of the zero-energy state $\ket{\Psi_0}$ in (\ref{aklt_state}) defined as follows
%\begin{equation}
	%\begin{split}
		%\ket{\Xi_-}&=\beta\sum_{\left\{\sigma_i\right\}_{i=1}^N}\sum_{b=1}^{N/2}\mathrm{Tr}\Big[B^{\sigma_1}C^{\sigma_2}\cdots M^{\sigma_{2b-1}\sigma_{2b}}\\&\times\cdots B^{\sigma_{N-1}}C^{\sigma_N}\Big]\ket{\sigma_1\cdots\sigma_N},
	%\end{split}
%\end{equation}  
%where $\beta$ is a normalization factor. Matrices $M^{\sigma_i\sigma_j}$ are defined as
%\begin{equation}
	%M^{\downarrow\downarrow}=\begin{pmatrix}
		%1 & 0\\ 0 & 1
	%\end{pmatrix},  M^{\downarrow\uparrow}=\begin{pmatrix}
	%\mu_1 & 0\\\mu_2 & 0
%\end{pmatrix}, M^{\uparrow\downarrow}=\begin{pmatrix}
%0 &0\\-\mu_2&\mu_1
%\end{pmatrix}
%\end{equation}
%with variational parameters $\mu_i\,\,(i=1, 2)$. The optimal $\ket{\Xi_-}$ is determined by minimizing the energy variance $\sigma^2(\mu_1, \mu_2)\equiv\braket{\Xi_-|H^2|\Xi_-}-\braket{\Xi_-|H|\Xi_-}^2$. The optimal values of $\mu_i$ for $N=20$ are $\mu_1\cong-1.120$ and $\mu_2\cong-6.80\times10^{-1}$ with the energy variance $\sigma^2(\mu_1,\mu_2)\cong2.846\times10^{-2}$. Although Ref.\cite{qmbs_aklt_vp} considers a superposition of $\ket{\Xi_-}$ and its translation $T_x\ket{\Xi_-}$ with a translation operator $T_x$, $\ket{\Xi_-}$ is already a reasonably good approximation of $\ket{-\epsilon}$ with $\left|\braket{-\epsilon|\Xi_-}\right|^2\cong6.204\times10^{-1}$. By changing $\mu_1\rightarrow-\mu_1$ we can also obtain the well-approximated scarred state $\ket{\Xi_+}$ for $\ket{\epsilon}$. Following (\ref{eq:zero_state}), we define the approximate zero-energy scarred state $\ket{\Xi_0}$ as 
%\begin{equation}\label{eq:zero_state_mps}
	%\ket{\Xi_0}=\beta_{\Xi}\left(1-(-1)^{N/2}\mathcal{C}\right)Q(\pi)\ket{\Xi_+},
%\end{equation} 
%where $\beta_\Xi$ is a normalization factor.

%This state approximates the exact scarred state with $E=0$ well with $\left|\braket{0|\Xi_0}\right|\cong5.717\times10^{-1}$ for $N=20$.
%We can construct the scar subspace as in Sec.\ref{subsec:E=0}. Here the scarred state $\ket{n}$ is defined as 
%\begin{equation}\label{eq:arroximate scar mps}
	%\ket{n}\equiv\begin{dcases}
		%\beta_n\left(Q^\dagger(\pi)\right)^n\ket{\Xi_0}&\quad(n>0)\\\ket{\Xi_0}&\quad(n=0)\\\beta_n\left(Q(\pi)\right)^{|n|}\ket{\Xi_0}&\quad(n<0)
	%\end{dcases}.
%\end{equation} 
%\begin{figure}
	%\centering
	%\includegraphics[width=.48\textwidth]{overlaps_from_mps_n_20.eps}
	%\caption{\label{fig:overlaps_from_mps}Overlap between the exact scarred states $\ket{\epsilon_n}$ (blue dots) or the $\mathbb{Z}_2$ state (red $\times$) and the approximate scarred states $\ket{n}$ for $N=20$ when we start from $\ket{\Xi_0}$ defined in (\ref{eq:zero_state_mps}).}
%\end{figure}
%Figure \ref{fig:overlaps_from_mps} shows our scarred states $\ket{n}$ can approximate the exact scarred state well. We note that $\ket{\pm1}$ is the better approximation of an adjacent scarred state than $\ket{\Xi_\pm}$ is.  
%\end{comment}

==> files_not_used/zero_energy_scarred_state.tex <==
Following the idea presented in Sec.~\ref{subsec:tos}, we first consider the reference state. Among several possibilities, we choose it to be the ``scarred" eigenstate with zero energy, corresponding to the red dot centered at the spectrum in Fig.\ref{fig:pbc_z2overlap_n_14}. We denote this scarred state by $\ket{\psi_0}$. Other states in the tower are denoted as $\ket{\psi_n}\,\,(n=-10\sim10 \text{ for } N=20)$. We define ``charge" operator $\mathcal{C}\equiv\sum_b\left(\dyad{L}_b-\dyad{R}_b\right)$, which counts $($\# of $L$s $-$ \# of $R$s$)$ of a given configuration. In order for $\ket{\psi_0}$ to be the zero energy state having a non-zero overlap with $\ket{\mathbb{Z}_2}$, it should be of a form
\begin{equation}\label{eq:exact scar state}
    \ket{\psi_0}=\sum_{k=0}^{N/2}(-1)^kc_k\ket{\psi_{N/2-2k}},
\end{equation}
where $c_k$ is a coefficient and $\ket{\psi_{N/2-2k}}$ satisfies
\begin{equation}\begin{split}
    &\braket{\psi_{N/2-2k}}=1,\\
    &\mathcal{C}\ket{\psi_{N/2-2k}}=\left(\frac{N}{2}-2k\right)\ket{\psi_{N/2-2k}}.
    \end{split}
\end{equation}
This is confirmed by realizing that $H$ changes the charge only by one. 

%\subsection{\label{subsec:island approximation}BCS Ansatz}
For the state $\ket{\psi_{N/2-2k}}$ in Eq.\eqref{eq:exact scar state} with small $k$, a vast majority of possible configurations contain only $O$s and $L$s (or $R$s), but do not contain all of three configurations. For example, $\ket{\psi_{N/2-2}}\,\,(k=1)$ must consist of two $O$s other than $L$s appearing $N/2-2$ times (such as $\ket{OLOLL\cdots}$). Assuming the scarred state is well approximated by such configurations, we define the ``creation" operator $a_L^\dag(b)$ as follows:
\begin{equation}\label{eq:creation islands}\begin{split}
    a_L^\dag(b)&=\left(1-\dyad{R}_{b-1}\right)\dyad{O}{L}_b\\&+\dyad{R}{O}_b\left(1-\dyad{L}_{b+1}\right)\\
    &=P_{2b-1}\sigma_{2b}^-P_{2b+1}+P_{2b}\sigma_{2b+1}^+P_{2b+2},
    \end{split}
\end{equation}
where $\sigma^+=\dyad{\uparrow}{\downarrow}$ and $\sigma^-=\dyad{\downarrow}{\uparrow}$. This operator creates $O$ on top of $L$s at a site $b$ in the block spin representation and $R$ at a site $b$ only when $O$ exists at a site $b+1$, increasing the charge by 1 in both cases. Similarly, we define the creation operator to create $O$ on top of $R$s as $a^\dag_R(b)=a_L(b)$.
%Within the islands configurations, this operator satisfies the following algebra:
%\begin{equation}
   % \begin{split}
    %    \left[a_b, a_b^\dag\right]&=\delta_{b,b'}\left(1-2n_b\right)\\
     %   \left\{a_b, a_b^\dag\right\}&=1\\
      %  \Big\{a_b, a_b\Big\}&=0,
    %\end{split}
%\end{equation}
%where $n_b=a_b^\dag a_b$ and $\left\{A, B\right\}\equiv AB+BA$ is anti-commutator. These relations are identical to those of spin $1/2$ algebra.
We also define two vacua as
\begin{equation}\begin{split}
    \ket{\Omega_L}&=\ket{\psi_{N/2}}=\ket{LL\cdots L}=\ket{\uparrow\downarrow\uparrow\downarrow\cdots}\\
    \ket{\Omega_R}&=\ket{\psi_{-N/2}}=\ket{RR\cdots R}=\ket{\downarrow\uparrow\downarrow\uparrow\cdots},
\end{split}
\end{equation}
which are $\ket{\mathbb{Z}_2}$ and its translation.

%Next we consider the PXP Hamiltonian. %If it acts on $\ket{b}\coloneqq a_b^\dag\ket{\Omega}$, we obtain
%\begin{equation}
    %H\ket{b}=\ket{\Omega}+\sum_{b'=1}^{N/2}a_{b'}^\dag\ket{b}.
%\end{equation}
%Note that due to the anticommutation relation of $a_b^\dag$, $a^\dag_b\ket{b}=0$. Therefore, the PXP Hamiltonian is roughly expressed as
%By comparing Eq.\eqref{eq:pxp lro} and Eq.\eqref{eq:creation islands}, one immediately gets
%\begin{equation}\label{eq:PXP island}
 %   H=\sum_{b=1}^{N/2}\left(a_b+a_b^\dag\right).
%\end{equation}
We consider the following ansatz that is a similar form to BCS wavefunction in superconductivity:
\begin{equation}
    \begin{split}
        \ket{\psi_{\rm{BCS}}}&=\frac{1}{\mathcal{N}}\left(\ket{\psi^L_{\rm{BCS}}}+(-1)^{N/2}\ket{\psi^R_{\rm{BCS}}}\right)\\
        \ket{\psi^L_{\rm{BCS}}}&=\exp\left[-\sum_lc(l)\sum_ba_L^\dag(b)a^\dag_L(b+l)\right]\ket{\Omega_L}\\
        \ket{\psi^R_{\rm{BCS}}}&=\exp\left[-\sum_lc(l)\sum_ba_R^\dag(b)a_R^\dag(b+l)\right]\ket{\Omega_R},
    \end{split}
\end{equation}
where $\mathcal{N}$ is a normalization factor and $c(l)$ is a parameter.
%\subsection{\label{subsec: dicke state}The scarred state as a superposition of the Dicke states}
%Since the operator $a_b$ satisfies the algebra of spin $1/2$, we can define collective angular momentum operators $J_+\equiv\sum_ba_b^\dag, J_-=J_+^\dag,$ and $J_z\equiv\sum_b\left(a_b^\dag a_b-1/2\right)$. Due to the constraint from Eq.\eqref{eq:exact scar state} that the number of islands must be even, the approximate scarred state, which we denote by $\ket{\psi_{\rm{island}}}$, should be a superposition of Dicke states, \begin{equation}
  %  \ket{\psi_{\rm{island}}}=\frac{1}{\mathcal{N}}\sum_{k=0}^{\lfloor N/4\rfloor}(-1)^kc_kJ_+^{2k}\ket{\Omega},
%\end{equation}
%where $\mathcal{N}$ is a normalization factor.
%Note that the vacuum state is an eigenstate of $J_z$ with an eigenvalue $-N/2$ and that \eqref{eq:PXP island} is written as $H_{\rm{island}}=J_++J_-=J_x$.
%We find the following simple ansatz shows a high overlap with the scarred state from exact diagonalization:
%\begin{equation}\label{eq:island scar}
 %   \ket{\psi_{\rm{island}}}=\frac{1}{\mathcal{N}}\exp\left[-\frac{J_+^2}{2(N-1)}\right]\ket{\Omega},
%\end{equation}
%where $\mathcal{N}$ is a normalization. We choose the coefficient $1/2(N-1)$ so that $H\ket{\psi_{\rm{island}}}$ does not contain terms with $\mathcal{C}=N/2-1$.

%We can further improve the fidelity by breaking homogeneity of the ansatz.
%\begin{equation}
 %   \ket{\psi'_{\rm{island}}}=\frac{1}{\mathcal{N}}\exp\left[-\sum_lc_l\sum_ba_b^\dag a_{b+l}^\dag\right]\ket{\Omega},
%\end{equation}
%where $\mathcal{N}$ is a normalization factor and $c_l$ is a coefficient which is determined to maximize the overlap $\left|\bra{\psi_0}\ket{\psi'_{\rm{island}}}\right|^2$.
We choose homogeneous coefficients $c(l)=(N/2-1)^{-1}$ so that $H\ket{\psi_{\rm{BCS}}}$ does not contain terms with $\mathcal{C}=\pm(N/2-1)$. This ansatz shows a remarkably high overlap with the exact scarred state which is $\left|\bra{\psi_0}\ket{\psi_{\rm{BCS}}}\right|^2\cong0.8095$ for $N=20$. We can further improve this overlap by optimizing the coefficients. It is found that the overlap even reaches $\left|\bra{\psi_0}\ket{\psi_{\rm{BCS}}}\right|^2\cong0.9254$ at optimal values for the same system size. 
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{overlaps_modified.pdf}
    \caption{Overlap with approximate scarred state within the island approximation and the scarred state from exact diagonalization.}
    \label{fig:overlaps}
\end{figure}
%When $N=20$, our ansatz shows $\left|\bra{\psi_0}\ket{\psi_{\rm{island}}}\right|^2\cong0.6801$ and $\left|\bra{\psi_0}\ket{\psi'_{\rm{island}}}\right|^2\cong0.7484$, which are quite high although our system is small-sized compared to other studies. 
We also point out that the coefficients at the optimal values do not deviate much from being homogeneous expect for $l=1$.%, suggesting that excitations tend to form a bound state.

Figure \ref{fig:overlaps} implies that overlaps scale exponentially, i.e., $\log\left|\bra{\psi_0}\ket{\psi_{\rm{BCS}}}\right|^2\cong e^{-\alpha N}$: for the homogeneous ansatz, $\alpha=0.01936$ and for the optimized wavefunction, $\alpha=0.006360$.
